The Spectrum of 1ES0229 + 200 and the Cosmic Infrared Background

We examine the effect of gamma-ray absorption by the extragalactic infrared radiation on intrinsic spectra predicted for 1ES0229+200 and compare our results with the observational data. We find agreement with our previous results on the shape of the IR spectral energy distribution (SED), contrary to the recent assertion of the HESS group. Our analysis indicates that 1ES0229+200 has a very hard intrinsic spectrum with a spectral index between 1.1 +/- 0.3 and 1.5 +/- 0.3 in the energy range between ~0.5 TeV and ~15 TeV. Under the assumptions that (1) the SED models of Stecker, Malkan & Scully (2006) are reasonable as derived from numerous detailed IR observations, and (2) spectral indexes in the range 1 < \Gamma < 1.5 have been shown to be obtainable from relativistic shock acceleration under the astrophysical conditions extant in blazar flares (Stecker, Baring & Summerlin 2007), the fits to the observations of 1ES0229+200 using our previous IR SEDs are consistent with both the IR and gamma-ray observations. Our analysis presents evidence indicating that the energy spectrum of relativistic particles in 1ES0229+200 is produced by relativistic shock acceleration, producing an intrinsic gamma-ray spectrum with index 1 < \Gamma < 1.5 and with no evidence of a peak in the SED up to energies ~15 TeV.

==> graphicx <==
%%
%% This is file `graphicx.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% graphicx.dtx  (with options: `package')
%% 
%% graphicx.dtx Copyright (C) 1994      David Carlisle Sebastian Rahtz
%%              Copyright (C) 1995 1996 1997 1999 David Carlisle
%%
%% This file is part of the Standard LaTeX `Graphics Bundle'.
%% It may be distributed under the terms of the LaTeX Project Public
%% License, as described in lppl.txt in the base LaTeX distribution.
%% Either version 1.0 or, at your option, any later version.
%%
\NeedsTeXFormat{LaTeX2e}[1995/12/01]
\ProvidesPackage{graphicx}
          [1999/02/16 v1.0f  Enhanced LaTeX Graphics (DPC,SPQR)]
\DeclareOption{unknownkeysallowed}
  {\PassOptionsToPackage\CurrentOption{keyval}}
\DeclareOption*{\PassOptionsToPackage\CurrentOption{graphics}}
\ProcessOptions
\RequirePackage{keyval,graphics}
\define@key{Gin}{bb}
           {\Gin@bboxtrue\Gread@parse@bb#1 \\}
\define@key{Gin}{bbllx}
           {\Gin@bboxtrue\Gin@defaultbp\Gin@llx{#1}}
\define@key{Gin}{bblly}
           {\Gin@bboxtrue\Gin@defaultbp\Gin@lly{#1}}
\define@key{Gin}{bburx}
           {\Gin@bboxtrue\Gin@defaultbp\Gin@urx{#1}}
\define@key{Gin}{bbury}
           {\Gin@bboxtrue\Gin@defaultbp\Gin@ury{#1}}
\define@key{Gin}{hiresbb}[true]{%
  \edef\Gread@BBox{%
    \@percentchar\@percentchar
    \csname if#1\endcsname HiRes\fi
    BoundingBox}}
\let\KV@Gin@natwidth\KV@Gin@bburx
\let\KV@Gin@natheight\KV@Gin@bbury
\define@key{Gin}{viewport}
           {\let\Gin@viewport@code\Gin@viewport\Gread@parse@vp#1 \\}
\define@key{Gin}{trim}
           {\let\Gin@viewport@code\Gin@trim\Gread@parse@vp#1 \\}
\def\Gread@parse@vp#1 #2 #3 #4 #5\\{%
  \Gin@defaultbp\Gin@vllx{#1}%
  \Gin@defaultbp\Gin@vlly{#2}%
  \Gin@defaultbp\Gin@vurx{#3}%
  \Gin@defaultbp\Gin@vury{#4}}%
\def\Gin@viewport{%
  \let\Gin@ollx\Gin@llx
  \let\Gin@olly\Gin@lly
  \let\Gin@ourx\Gin@urx
  \let\Gin@oury\Gin@ury
  \dimen@\Gin@llx\p@\advance\dimen@ \Gin@vurx\p@
                      \edef\Gin@urx{\strip@pt\dimen@}%
  \dimen@\Gin@lly\p@\advance\dimen@ \Gin@vury\p@
                      \edef\Gin@ury{\strip@pt\dimen@}%
  \dimen@\Gin@llx\p@\advance\dimen@ \Gin@vllx\p@
                      \edef\Gin@llx{\strip@pt\dimen@}%
  \dimen@\Gin@lly\p@\advance\dimen@ \Gin@vlly\p@
                      \edef\Gin@lly{\strip@pt\dimen@}}
\def\Gin@trim{%
  \let\Gin@ollx\Gin@llx
  \let\Gin@olly\Gin@lly
  \let\Gin@ourx\Gin@urx
  \let\Gin@oury\Gin@ury
  \dimen@\Gin@llx\p@\advance\dimen@ \Gin@vllx\p@
                      \edef\Gin@llx{\strip@pt\dimen@}%
  \dimen@\Gin@lly\p@\advance\dimen@ \Gin@vlly\p@
                      \edef\Gin@lly{\strip@pt\dimen@}%
  \dimen@\Gin@urx\p@\advance\dimen@ -\Gin@vurx\p@
                      \edef\Gin@urx{\strip@pt\dimen@}%
  \dimen@\Gin@ury\p@\advance\dimen@ -\Gin@vury\p@
                      \edef\Gin@ury{\strip@pt\dimen@}}
\let\Gin@vllx\Gin@llx\let\Gin@vlly\Gin@llx
\let\Gin@vurx\Gin@llx\let\Gin@vury\Gin@llx
\define@key{Gin}{angle}
           {\Gin@esetsize
            \@tempswatrue
            \edef\@tempa{\toks@{\noexpand\Gin@erotate{#1}{\the\toks@}}}%
            \@tempa}
\define@key{Gin}{origin}[c]{%
  \def\Gin@erotate{\Grot@box@kv[origin=#1]}}
\define@key{Gin}{width}{\def\Gin@ewidth{#1}}
\define@key{Gin}{height}{\def\Gin@eheight{#1}}
\define@key{Gin}{totalheight}{%
  \def\Gin@eresize{\totalheight}\def\Gin@eheight{#1}}
\define@key{Gin}{keepaspectratio}[true]{%
  \lowercase{\Gin@boolkey{#1}}{iso}}
\define@key{Gin}{scale}{%
  \if@tempswa
    \edef\@tempa{\toks@{\noexpand\Gscale@box{#1}[#1]{\the\toks@}}}%
    \@tempa
  \else
    \def\Gin@req@sizes{%
      \def\Gin@scalex{#1}\let\Gin@scaley\Gin@exclamation
      \Gin@req@height\Gin@scalex\Gin@nat@height
      \Gin@req@width\Gin@scalex\Gin@nat@width}%
  \fi
  \@tempswatrue}
\define@key{Gin}{draft}[true]{%
  \lowercase{\Gin@boolkey{#1}}{draft}}
\define@key{Gin}{clip}[true]{%
  \lowercase{\Gin@boolkey{#1}}{clip}}
\define@key{Gin}{type}{%
  \def\Ginclude@graphics##1{%
    \begingroup
    \def\Gin@base{##1}%
    \edef\@tempa{{#1}{\Gin@eread}{\Gin@ecom{##1\Gin@eext}}}%
    \expandafter\Gin@setfile\@tempa
    \endgroup}}
\define@key{Gin}{ext}{\def\Gin@eext{#1}}
\let\Gin@eext\@empty
\define@key{Gin}{read}{%
 \def\Gin@eread{#1}%
 \def\@tempa{*}\ifx\@tempa\Gin@eread\def\Gin@eread{\Gin@eext}\fi}
\let\Gin@eread\@empty
\define@key{Gin}{command}{\def\Gin@ecom##1{#1}}
\let\Gin@ecom\@firstofone
\def\Gin@boolkey#1#2{%
  \csname Gin@#2\ifx\relax#1\relax true\else#1\fi\endcsname}
\def\Gin@eresize{\height}
\def\Gin@esetsize{%
  \let\@tempa\Gin@exclamation
  \if@tempswa
    \edef\@tempa{\toks@{\noexpand
             \Gscale@@box\noexpand\Gin@eresize
              {\Gin@ewidth}{\Gin@eheight}{\the\toks@}}}%
    \@tempa
  \else
    \ifx\Gin@ewidth\@tempa
      \ifx\Gin@eheight\@tempa
      \else
         \let\Gin@@eheight\Gin@eheight
         \def\Gin@req@sizes{%
           \Gscale@div\Gin@scaley\Gin@@eheight\Gin@nat@height
           \let\Gin@scalex\Gin@exclamation
           \setlength\Gin@req@height\Gin@@eheight
           \Gin@req@width\Gin@scaley\Gin@nat@width}%
      \fi
    \else
      \ifx\Gin@eheight\@tempa
         \let\Gin@@ewidth\Gin@ewidth
         \def\Gin@req@sizes{%
           \Gscale@div\Gin@scalex\Gin@@ewidth\Gin@nat@width
           \let\Gin@scaley\Gin@exclamation
           \setlength\Gin@req@width\Gin@@ewidth
           \Gin@req@height\Gin@scalex\Gin@nat@height}%
      \else
         \let\Gin@@ewidth\Gin@ewidth
         \let\Gin@@eheight\Gin@eheight
         \def\Gin@nosize##1{%
           \KV@Gin@natwidth\Gin@@ewidth
           \KV@Gin@natheight\Gin@@eheight}%
         \def\Gin@req@sizes{%
           \Gscale@div\Gin@scalex\Gin@@ewidth\Gin@nat@width
           \Gscale@div\Gin@scaley\Gin@@eheight\Gin@nat@height
           \ifGin@iso
             \ifdim\Gin@scaley\p@>\Gin@scalex\p@
               \let\Gin@scaley\Gin@scalex
             \else
               \let\Gin@scalex\Gin@scaley
             \fi
           \fi
           \Gin@req@width\Gin@scalex\Gin@nat@width
           \Gin@req@height\Gin@scaley\Gin@nat@height}%
       \fi
     \fi
  \fi
  \let\Gin@ewidth\Gin@exclamation
  \let\Gin@eheight\Gin@ewidth}
\newdimen\Gin@req@height
\newdimen\Gin@req@width
\let\Gin@outer@scalex\relax
\let\Gin@outer@scaley\relax
\let\Gin@angle\relax
\let\Gin@ewidth\Gin@exclamation
\let\Gin@eheight\Gin@ewidth
\def\Gin@scalex{1}
\let\Gin@scaley\Gin@exclamation
\def\Gin@i{%
 \def\Gin@req@sizes{%
   \Gin@req@height\Gin@nat@height
   \Gin@req@width\Gin@nat@width}%
 \@ifnextchar[\Gin@ii{\Gin@ii[]}}
\def\Gin@ii[#1]#2{%
    \def\@tempa{[}\def\@tempb{#2}%
    \ifx\@tempa\@tempb
      \def\@tempa{\Gin@iii[#1][}%
      \expandafter\@tempa
    \else
     \begingroup
       \@tempswafalse
       \toks@{\Ginclude@graphics{#2}}%
       \setkeys{Gin}{#1}%
       \Gin@esetsize
       \the\toks@
     \endgroup
     \fi}
\def\rotatebox{%
  \@ifnextchar[\Grot@box@kv\Grot@box@std}
\def\Grot@box@std#1#2{%
  \Grot@setangle{#1}%
  \setbox\z@\hbox{{#2}}%
  \Grot@x\z@
  \Grot@y\z@
  \Grot@box}
\def\Grot@box@kv[#1]#2#3{%
  \@begin@tempboxa\hbox{#3}%
    \Grot@x\width \divide\Grot@x\tw@
    \Grot@y\height \advance\Grot@y-\depth \divide\Grot@y\tw@
    \setkeys{Grot}{#1}%
    \setbox\z@\box\@tempboxa
    \Grot@setangle{#2}%
    \Grot@box
  \@end@tempboxa}
\define@key{Grot}{origin}[c]{%
 \@tfor\@tempa:=#1\do{%
    \if l\@tempa \Grot@x\z@\else
    \if r\@tempa \Grot@x\width\else
    \if t\@tempa \Grot@y\height\else
    \if b\@tempa \Grot@y-\depth\else
    \if B\@tempa \Grot@y\z@\fi\fi\fi\fi\fi}}
\define@key{Grot}{x}{\setlength\Grot@x{#1}}
\define@key{Grot}{y}{\setlength\Grot@y{#1}}
\define@key{Grot}{units}{%
  \def\Grot@setangle##1{%
  \dimen@##1\p@
  \dimen@ii#1\p@
  \divide\dimen@ii360\relax
  \divide\dimen@\dimen@ii
  \edef\Grot@angle{\number\dimen@}}}
\let\Gin@erotate\Grot@box@std
\endinput
%%
%% End of file `graphicx.sty'.
